Principles and Practices of Large-Scale Code Analysis at Ant Group: A Data- and Logic-Oriented Approach

Large-scale software development requires dynamic and multifaceted static code analysis that extends beyond the capabilities of traditional tools. Existing tools like CodeQL lack cross-language analysis capabilities and can be time-consuming and resource-intensive. We present CodeFuse-Query, a data system tailored for large-scale code analysis. First, CodeFuse-Query adopts a Logic-Oriented Computation Design, employing Datalog with a two-tiered schema, COREF, to convert source code into data facts, and Godel to express complex analysis tasks in logical terms. Furthermore, CodeFuse-Query adopts a Domain-Optimized System Design. This approach optimizes resource utilization, prioritizes data reusability, applies incremental code extraction, and introduces task-type characteristics specifically for code changes, underscoring its domain-optimized design. We present empirical results demonstrating CodeFuse-Query's robustness, scalability, and efficiency in large-scale real-world scenarios at Ant Group, where it serves as a core static analysis infrastructure. Deployed in production environments, CodeFuse-Query processes up to 10 billion lines of code daily across more than 300,000 distinct analysis tasks. CodeFuse-Query has been open-sourced.

==> detaileddesign.tex <==
In this section, we delve into our distinctive approach for modeling data derived from source code. Given the inherent complexities of static source code analysis, the representation of source code becomes a crucial determinant of the success of our methodology.

A myriad of considerations and obstacles must be navigated during this endeavor. The first challenge stems from the absence of a standardized method for transforming source code into a data-friendly format, pushing us to devise a unique strategy suited to our specific needs.

Furthermore, source code serves as a trove of dense information, both semantically and syntactically. This necessitates the exercise of careful discernment in choosing what details to encapsulate and what to leave out. Such decisions should be guided by an assessment of the relevance and utility of the information in question.

Our platform, designed for comprehensive code analysis, aims to preserve as much source code information as possible without diluting the original data. This ensures that we can support a wide array of analyses by extracting required data on an ad-hoc basis. In essence, our design is not restricted to specific tasks but is flexible and adaptable to a variety of analytical needs.

Our system's efficiency is contingent on the initial extraction and persistent storage of the source code. The scale of this process can potentially strain storage resources. Therefore, it becomes imperative to ensure that the stored code data is optimized for compactness, thus mitigating the risk of excessive resource utilization.





\subsection{Background: Source Code Representation}

\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{resources/code_representation.pdf}
\caption{A typical code representation dependency diagram}
\label{fig:code_rep}
\end{figure}

Source code can be represented in numerous ways, with the most prevalent and standardized methods being those utilized in compilers and static analyzers.

Among these, the abstract syntax tree (AST) is the most recognized representation. Used extensively by compilers for parsing code, the AST captures comprehensive syntax and grammar information of the source code.

Other frequently used representations include the Abstract Semantic Graph (ASG), which incorporates crucial semantic information into the graph, and the Program Dependency Graph (PDG), which facilitates the analysis of data and control dependencies within the code.

From the graph, it is evident that by recording the tokens and AST information of a source code, we can extract the complete source information without needing the actual source code files. Additionally, with the AST at our disposal, all other information can be recovered, albeit at varying costs.

In conclusion, given the widespread use of this information by numerous analyzers, our objective is to devise a methodology that can retain all this data. This approach will enable the data to be queried as and when required, thereby enhancing the utility and accessibility of the stored information.


\gang{Compare with other representations such as cpg, uast}

\gang{Compare with Codeql}

\gang{talk about the openness/extensible of the current design}


\subsection{Two-tiered Data Modelling of Source Code}

\begin{figure*}[h]
\centering
\includegraphics[width=\textwidth]{resources/modeldesign.pdf}
\caption{Two-tiered Design of Code Data Model}
\label{fig:code_data_model}
\end{figure*}

Given the complexity of encapsulating all source code information in a single database, we have devised a novel two-tiered modeling strategy. Figure~\ref{fig:code_data_model} shows the conceptual idea of the data modelling.

The first step in our process involves extracting the source code and storing it within a database. This process is represented by our Layer 1 model, which consists of approximately a hundred tables for each programming language.

Subsequently, this initial database is utilized to retrieve more semantic information in memory, functioning similarly to views in traditional relational databases. This ensures that all queries operate on the second layer data, which is managed uniformly.

Our first layer is dedicated to storing AST information within efficiently designed tables. The primary consideration in the table design is to avoid storing duplicate information in the database, while ensuring that other information can be recomputed as needed. The resulting database is designed for persistent storage. For instance, a typical Java repository with approximately 500K lines of code may occupy around 800MB in the database. Even after compression, the size remains substantial for a static analysis task. Given that we need to analyze multiple versions of the same repository, the database size could significantly increase system overhead.

For the second layer, we employ a datalog intentional schema for modeling. The intentional schema is defined by datalog predicates and linked together to establish the execution plan for each detailed information. Typical facts (e.g., a class's qualified name) are calculated by jointly analyzing multiple tables from the Layer 1 model (e.g., by collectively analyzing the class identity table, token name table, and so on).

It's important to note that in our system, the Layer 2 model is not persisted; rather, it is computed as needed. This approach is due to the impracticability of storing all information on disk. For example, precomputing and expanding all the information for a typical Java repository would require approximately four hours and 30GB of disk space.

In the context of Datalog—a declarative logic programming language used for deductive databases—our Layer 1 model is known as the "Extensional Database" or EDB\cite{Ullman1989}. The EDB is comprised of ground facts, or basic information, that are available before computation commences. Essentially, the EDB forms the base facts upon which further reasoning and computations are performed.

In contrast, the Layer 2 schema, which is formulated using a Datalog Domain-Specific Language (DSL), is referred to as the "Intensional Database" or IDB. The IDB is comprised of facts that are not initially present, but are derived or inferred from the EDB facts through the application of rules. The IDB, thus, represents the more complex, derived facts that emerge from the reasoning process.

In summary, our approach, when combined with user-specific queries, enables us to interconnect all data and encapsulate all static analysis tasks as simple Datalog computation tasks. This two-tiered method facilitates an efficient and effective way to manage and analyze source code information by distinguishing between base facts (EDB) and derived facts (IDB).

\subsection{Extraction of Tier-1 Model}

The crux of our two-tiered modeling approach is the design of the extractor for the Tier-1 model. Essentially, the extractor functions as a source code parser, and we have devised one for each distinct language and configuration. This decision bears significant engineering advantages. For instance, it's far simpler to parse Go using Go, rather than striving for a universal parser for all languages.

Our parser design is governed by the following practical considerations:

Independence from build processes: Typically, most languages involve a build process and associated build tools, such as Maven for Java, Bazel for C++, and so forth. However, we've ensured that our extractor doesn't rely on any build process. This choice is rooted in the reality that build processes are often unreliable and brittle, and even maintaining a robust build process can pose a significant challenge for large organizations. Incorporating the build system into our own could further exacerbate these challenges. By steering clear of build processes, we enhance the maintainability and ease of debugging for our system. The downside is that this might result in the loss of some information, particularly for C family languages, which have a dedicated preprocessing stage of code compilation. If the build process isn't captured, retrieving the preprocessing arguments becomes impossible, making it difficult to understand the true semantics of the code. Techniques such as fuzzy parsing could offer some respite in such scenarios.

Language-specific extractors: Our approach involves crafting an extractor for each distinct language separately.

Expertise-driven design: The design of the extraction stage is a balancing act between storage space and computational efficiency. It requires expert experience and knowledge to decide what should be included at this stage since some information could be calculated later or during the extraction stage itself. For instance, for the Java language, we rely on the parser to generate reference information (symbol linkage), as the Java resolver we use is highly optimized and considerably less computationally intensive than using Datalog for subsequent computations.

Our two-tiered approach allows us to formulate a standardized engineering process that can be scaled across a team, enabling us to model multiple different languages simultaneously.

Developing the model and extractor requires extensive engineering effort. Table~\ref{tbl:coref_nodes} provides a glimpse into the current state of our data modeling work by outlining the number of nodes in each data model. In practice, an engineer should scrutinize each node of the language parser and meticulously design each entity of the language model.

\xiaoheng{please keep the language name consistent}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\begin{tabular}{llrrl}
\multicolumn{1}{c}{\cellcolor[HTML]{4472C4}}                           & \multicolumn{1}{c}{\cellcolor[HTML]{4472C4}}                        & \multicolumn{2}{l}{\cellcolor[HTML]{4472C4}No. of Nodes}                                                              &  \\
\multicolumn{1}{c}{\multirow{-2}{*}{\cellcolor[HTML]{4472C4}Language}} & \multicolumn{1}{c}{\multirow{-2}{*}{\cellcolor[HTML]{4472C4}State}} & \multicolumn{1}{c}{\cellcolor[HTML]{4472C4}Layer-1 Model} & \multicolumn{1}{c}{\cellcolor[HTML]{4472C4}Layer-2 Model} &  \\
Java                                                                   & Mature                                                              & 157                                                       & 482                                                       &  \\
XML                                                                    & Mature                                                              & 12                                                        & 27                                                        &  \\
TS/JS                                                                  & Mature                                                              & 392                                                       & 574                                                       &  \\
OC/C++                                                                 & Beta                                                                & 53                                                        & 109                                                       &  \\
Go                                                                     & Beta                                                                & 38                                                        & 263                                                       &  \\
Python                                                                 & Beta                                                                & 55                                                        & 120                                                       &  \\
Swift                                                                  & Beta                                                                & 248                                                       & 679                                                       &  \\
SQL                                                                    & Beta                                                                & 750                                                       & 2552                                                      &  \\
Properties                                                             & Beta                                                                & 9                                                         & 11                                                        & 
\end{tabular}
\caption{Current Code Model Statistics}
\label{tbl:coref_nodes}
\end{table}



==> godel.tex <==
\subsection{The Imperatives for a DSL}
In this section, we delve into the role and design rationale of the \DatalogName domain-specific language (DSL), a pivotal component of our big data analytic system. The imperative for a DSL like \DatalogName arises from several fundamental challenges in the realm of code analysis, a field that has burgeoned in complexity and diversity with the advent of big data. Some of these challenges have been discussed in the Background and Challenge section.

\textbf{Challenge 1: User-Friendly and Controlled Interface (Interface Challenge)}\\
The first challenge, the Interface Challenge, is rooted in the broader issue of Problem Complexity and Dynamism as outlined in the Background and Challenge section. As previously discussed, the diverse nature of tasks and their unique requirements necessitate an interface that is both user-friendly and manageable. Traditionally, the design of interfaces for code analysis tasks has been a delicate balance between user-friendliness and control. However, as the scale and complexity of these tasks burgeon in the era of big data, maintaining this balance becomes increasingly crucial. An ideal interface should be intuitive enough for users to articulate their tasks effectively, yet also limit potentially disruptive operations, such as the creation of infinite loops that could jeopardize the entire system. \DatalogName's design addresses this Interface Challenge by offering an easy-to-master interface that also circumscribes the scope of user operations to uphold system stability.

\textbf{Challenge 2: Efficient Code Structure and Computation Modeling (Modeling Challenge)}\\
The Modeling Challenge is an extension of the Diversity of Analysis Targets and Scalability and Speed challenges discussed earlier.
Given the colossal amounts of data and the intricate code structures intrinsic in big data analysis, traditional methods that rely on persisting all data are no longer sustainable. The Modeling Challenge is met by \DatalogName's unique on-the-fly, in-memory computation capabilities, offering a resilient solution for managing and maintaining these complex structures without the necessity for complete data persistence.

\textbf{Challenge 3: Sustainable and Adaptable Code Information Modeling (Adaptability Challenge)}\\
The Adaptability Challenge relates back to the importance of High Maintainability and Interoperability as discussed in the Background and Challenge section.
As programming and configuration languages evolve and their standards shift, so too must the methods for modeling source code. \DatalogName has been designed with this Adaptability Challenge in mind, enabling it to adjust to different schemas and standards, thereby ensuring the sustainability of source code information and maintaining compatibility with various tools and languages.

\textbf{Challenge 4: Superior Computational Efficiency (Efficiency Challenge)}\\
The Efficiency Challenge is a direct link to the Scalability and Speed and Resource Constraints and Variability challenges identified in the Background and Challenge section.
The escalating scale of code analysis tasks in big data analytics necessitates superior computational efficiency. Tasks often entail extensive graph traversal, property analysis, recursive analysis, and dataflow analysis, all of which are computationally intensive. The large scale of big data can easily trigger NP-Hard problems, making efficiency a necessity rather than a luxury. \DatalogName's design considers this Efficiency Challenge, optimizing for computational efficiency to handle the rigors of big data code analysis.


The aforementioned imperatives collectively underscore the need for a uniform solution that can address all these challenges in a coherent, integrated manner. This is where the \DatalogName system truly excels. By designing a DSL specifically tailored to the needs of big data code analysis, \DatalogName provides a holistic solution that attends to user interface design, code structure modeling, computational efficiency, and system integration. 

Although the comprehensive implementation and design details of \DatalogName are beyond the scope of this paper, we will discuss several key design choices that underscore its essential role in our large-scale code analysis system. 


\subsection{Underlying Computation Model: Datalog}

The computational foundation of each \DatalogName program is rooted in Datalog, which implies that \DatalogName shares the same computational model as a typical Datalog program. Datalog\cite{Ceri1989}, a declarative logic language\cite{logicprogramming}, provides an abstraction layer that allows users to focus on defining their computations while abstracting away the intricate details of execution and evaluation.

Datalog is a logic language\cite{logicprogramming} that offers an intuitive and user-friendly approach to algorithm specification. Its syntax and structure align closely with the natural flow of pseudo code, promoting ease of writing and maintenance. Datalog also supports complex queries, recursion, and logical reasoning, making it an ideal choice for static code analysis.

Let's consider a more comprehensive example that describes a Datalog program for calculating the ancestor-class information of classes. In this example, we have two predicates: `parent`, which captures the immediate parent-child relationship between classes, and `ancestorclass`, which captures the ancestor-descendant relationship. 

\begin{verbatim}
parent(a, b) :- class(a), 
                extends(a, b), 
                class(b).

ancestorclass(a, b) :- parent(a, b).

ancestorclass(a, c) :- parent(a, b), 
                        ancestorclass(b, c).
\end{verbatim}

In this program, the `:-` symbol is used for predicate definition, and `,` represents a logical AND. The first rule defines the `parent` predicate based on the `class` and `extends` predicates. The second rule captures the immediate parent-child relationship in the `ancestorclass` predicate. The third rule defines the recursive case for the `ancestorclass` predicate, allowing it to capture multi-level ancestor-descendant relationships.

The underlying computation model of Datalog is a specialized form of relational algebra, meaning Datalog programs essentially perform logical computations among facts. This model also supports recursive computation\cite{bancilhon1986recursive}, a feature frequently needed in static code analysis. Many source code analysis tasks, like determining all methods reachable from a given method or identifying all child classes of a given class, require the computation of a fixpoint, which can be naturally expressed in Datalog\cite{Bancilhon1986}.

One of the key strengths of Datalog—and by extension, \DatalogName—is the computational efficiency it brings to the table. This efficiency stems from several inherent features of Datalog.

Firstly, Datalog programs have an underlying execution plan that can be optimized using various optimization algorithms. This means that the actual computations performed during the execution of a Datalog program can be streamlined and organized in a way that minimizes computational resources and time. 

Secondly, Datalog has built-in safeguards that guarantee the termination of its programs. This feature not only eliminates the risk of infinite loops but also ensures that all computational resources are used effectively, without being wasted on non-terminating tasks. As a result, users can confidently execute their tasks with the assurance that the system will reliably return a result.

Thirdly, Datalog is inherently set-oriented. This means it operates on sets of data at a time, rather than individual data points. This set-oriented operation allows Datalog to perform operations like joins and projections more efficiently than point-oriented languages, making it well-suited for big data applications.

Lastly, Datalog's declarative nature allows it to efficiently handle complex queries and recursive computations. Since users only need to specify what they want, rather than how to compute it, Datalog can automatically choose the most efficient execution strategy. This feature, combined with the support for recursive computation, makes Datalog extremely efficient for tasks that involve complex logical reasoning, such as many static code analysis tasks.

These features collectively make Datalog—and therefore, \DatalogName—an efficient and powerful tool for big data code analysis. With its optimized execution plans, guaranteed termination, set-oriented operations, and efficient handling of complex queries, Datalog provides a robust and computationally efficient foundation for \DatalogName.



\subsection{Interlinking the \DatalogName Model with Tier-1 and Tier-2 Data Models}

We now pivot to illustrate how the \DatalogName model interfaces with the Tier-1 and Tier-2 data models. This connection is elucidated in Figure~\ref{fig:query_to_db}.

In the initial block, a user constructs a query employing a series of high-level language features, such as types, classes, functions, and modules. These high-level features represent user-oriented concepts, designed for intuitive understanding. Additionally, the \DatalogName language introduces syntactic sugar, thus simplifying the code-writing process for users.

These high-level features are defined and implemented in \DatalogName, which offers comprehensive algorithms and computational strategies to calculate the high-level information demanded by user queries. Within the data model context, this is referred to as the Tier-2 data model. Worth noting is that this level functions more as an abstract description or view of how information is computed, rather than the actual computation and persistence. This unique characteristic allows for the generation of a specific execution plan for each query, thereby enhancing performance.

Ultimately, the \DatalogName query is transformed into computations conducted among the foundational layer of predicates, where the extensional facts (EDB) are supplied in runtime. This transformation elucidates the interconnection between the query, the library, and the data, addressing the Interface, Modeling, Adaptability, and Efficiency.


\begin{figure}[ht]
  \centering
  \includegraphics[width=0.5\textwidth]{resources/query_to_db.pdf}
  \caption{Illustration of the interconnection between user query, tier-1 and tier-2 code models.}
  \label{fig:query_to_db}
\end{figure}


\subsection{Rich and highlevel program features}
A key strength of the \DatalogName language lies in its rich set of high-level program features, which make it particularly well-suited for handling complex code analysis tasks in a big data environment.

First and foremost, \DatalogName provides a high degree of abstraction that enables users to describe complex algorithms in a concise and intuitive manner. By leveraging the underlying Datalog model, \DatalogName allows users to define high-level predicates and rules that can encapsulate complex logic. The high-level abstraction also simplifies code maintenance and revision, as changes in the underlying logic can be made without altering the overall program structure.

\DatalogName also boasts a robust type system, which enhances both the expressiveness and safety of the \DatalogName programs. With the ability to define complex data types and enforce type checks, \DatalogName ensures the integrity of the data and prevents type-related errors, a critical feature in a big data environment where even a minor error can lead to significant issues due to the large volume of data.

Another major feature of \DatalogName is its support for modularity. \DatalogName programs can be organized into modules, each encapsulating a specific aspect of the code analysis task. This modularity facilitates code reuse, enhances readability, and simplifies maintenance by enabling separate development, testing, and revision of individual modules.

Moreover, \DatalogName supports a variety of control structures, including recursion, conditionals, and looping constructs. This feature set allows \DatalogName to express a wide range of algorithms, from simple iterative tasks to complex recursive computations, thereby increasing its versatility.

Finally, \DatalogName stands out for its seamless integration with external systems and data sources. \DatalogName programs can interact with databases, files, and web services, allowing them to fetch, process, and store data as required. This capability is crucial in a big data context, where data sources are diverse and distributed.

For instance, consider our Java library modeling code, which comprises approximately 60,000 lines of \DatalogName code. If we were to translate this into Datalog, it would require around 350,000 lines of code — a significant increase in complexity. The introduction of high-level features in \DatalogName contributes substantially to the manageability of large-scale analysis code, demonstrating \DatalogName's efficiency and compactness compared to traditional Datalog.

In summary, the rich high-level features of the \DatalogName language, combined with its powerful underlying computation model, make it an ideal tool for complex code analysis tasks in big data analytics. Its user-friendly syntax, robust type system, modularity, diverse control structures, and seamless external integration collectively contribute to its effectiveness and efficiency, allowing it to handle the challenges of big data code analysis with remarkable ease.


\subsection{Support of User-Defined Functions (UDFs) and Foreign Functions}

While Datalog is a powerful language, its restrictions can limit its capabilities in certain scenarios. There are algorithms, for instance, that are difficult or even impossible to describe within the confines of Datalog. To address this, we have incorporated support for User-Defined Functions (UDFs) in \DatalogName, enabling the inclusion of components written in C or C++ languages. This allows us to support computations like MD5 hashing or regular expression searches, which are challenging to express in Datalog.

The support for UDFs effectively makes \DatalogName a Turing-complete language, expanding its capacity to solve a broader set of computational problems. However, this also comes at the cost of sacrificing some of the predictability inherent in \DatalogName programs. This trade-off is a practical consideration, and thus the selection and management of UDFs require careful attention. 

To maintain system stability, the platform currently supports only a selective set of functions, and these are centrally managed by the platform team. Although it is technically feasible, we do not currently allow users to define their own UDFs. This approach helps to prevent overuse or misuse of this feature, which could potentially compromise the integrity of the entire platform. Hence, while UDFs enable a wider range of functionality in \DatalogName, their use is carefully managed to maintain the overall reliability and performance of the platform.

\subsection{Ample Opportunities for Optimization}

Given the computationally intensive nature of static code analysis, optimizing execution to minimize CPU and memory usage is not just beneficial, but often essential. 

\DatalogName provides several opportunities for such optimization. Each \DatalogName program can be converted into an execution plan, simplifying the computation process and presenting potential areas for optimization. Through the application of various optimization algorithms\cite{Bancilhon1986}, we can significantly reduce the complexity of a typical query. For example, as shown in Figure~\ref{fig:exeuction_plan} we have been able to reduce an analysis from 2832 computation nodes down to a mere 17, while still achieving the same results. 

\begin{figure*}[ht]
  \centering
  \includegraphics[width=\textwidth]{resources/exeuction_plan.pdf}
  \caption{An example showing the optimization in execution plan level}
  \label{fig:exeuction_plan}
\end{figure*}

In addition to program-level optimization, the design of \DatalogName also facilitates system-level optimization. For instance, we can cache "hot" facts - data points that are frequently computed and referenced by common queries. This reduces the time and resources spent on repeatedly computing the same facts. 

Furthermore, by analyzing usage patterns within our system, we can anticipate and precompute certain facts even before a query is made. This proactive approach enhances the overall efficiency of the system, ensuring that it can handle the demands of large-scale code analysis tasks with minimal resource consumption.



